Path association rule mining

Graph association rule mining is a data mining technique used for discovering regularities in graph data. In this study, we propose a novel concept, {\it path association rule mining}, to discover the correlations of path patterns that frequently appear in a given graph. Reachability path patterns (i.e., existence of paths from a vertex to another vertex) are applied in our concept to discover diverse regularities. We show that the problem is NP-hard, and we develop an efficient algorithm in which the anti-monotonic property is used on path patterns. Subsequently, we develop approximation and parallelization techniques to efficiently and scalably discover rules. We use real-life graphs to experimentally verify the effective

==> algorithms/frequentattribute.tex <==
 \begin{algorithm}[!t] 
	\caption{Frequent attribute discovery}	\label{alg:frequentattribute}
		\DontPrintSemicolon
			    %\SetKwInOut{Input}{input}
	            %\SetKwInOut{Output}{output}
	             \SetKwFunction{Expand}{Expand}
	            %\Input{Graph $\graph$, min support $\minsup$}
              
              ${\mathcal C} \gets \forall a \in \attributes$\\
              ${\pathpatterns}_0 \gets \varnothing$\\
              \While{${\mathcal C} \neq \varnothing$}{
            %   \For{$c \in \mathcal C$}{
            %   $i \gets 0$\\
            %   \For{$v \in V$}{
            %         \If{$A(v) \subseteq c$}{
            %             $i \gets i+1$\\
            %         }
            %       }
            %       \If{$i > \minsup$}{
            %          $F \gets F \cup c$
            %       }
            %       }
                  ${\pathpatterns}_0 \gets {\pathpatterns}_0 \cup$ {\sf Discovery(${\mathcal C}, \graph, \minsup$)}\\
                  ${\mathcal C} \gets$ {\sf GenerateCandidate($\attributes_S$)}\\
              }
               \For{$\elabel \in \elabels$}{
                    $(\edges_F,\attributes_T)  \gets$ {\sf MatchedEdges($\elabel$)}\\
               }
              %{\bf end procedure}
\end{algorithm}


==> algorithms/kleenepathdiscovery.tex <==
\begin{algorithm}[!t] 
	\caption{Frequent Kleene path pattern discovery}	\label{alg:kleenepathpattern}
		\DontPrintSemicolon
			    \SetKwInOut{Input}{input}
	            \SetKwInOut{Output}{output}
	             \SetKwFunction{Expand}{Expand}
	          %  \Input{Graph $\graph$, min support $\minsup$, length $\minlen$}
              ${\pathpatterns}^* \gets \varnothing$\\
                 $\vertices_T \gets${\sf BFS($\elabels_F, \graph, \minlen$)}\\
              
              ${\mathcal C} \gets \forall p$ compuated by $\elabels_F, \attributes_T, \pathpatterns_0$\\
              \While{${\mathcal C} \neq \varnothing$}{
            %   \For{$c \in \mathcal C$}{
            %   $i \gets 0$\\
            %   \For{$v \in V$}{
            %         \If{$A(v) \subseteq c$}{
            %             $i \gets i+1$\\
            %         }
            %       }
            %       \If{$i > \minsup$}{
            %          $F \gets F \cup c$
            %       }
            %       }
                  ${\pathpatterns}^* \gets {\pathpatterns}^* \cup$ {\sf Discovery(${\mathcal C}, \graph, \minsup, \vertices_T$)}\\
                  ${\mathcal C} \gets$ {\sf HorizontalExtend(${\pathpatterns}^*$)}\\
                }
            %   \For{$c, c' \in \mathcal C$}{
            %   $i \gets 0$\\
            %       \For{$\elabel \in \mathcal N$}{
                  
            %         \For{$v \in V$}{
            %             \If{$A(v) \subseteq c$ and $A(v')$}{
            %                 $i \gets i+1$\\
            %             }
            %           }
                     
            %           \If{$i > \minsup$}{
            %              $F \gets F \cup c$
            %           }
            %       }
            %   }
                    
            %   \While{1}{
            %   ${\mathcal C} \gets$ {\sf GenerateCandidate($F$)}\\
            %   \If{$\mathcal C = \varnothing$}{\bf{break}}
              
            %   \For{$v \in V$}{
            %      \If{$v.F \subseteq c$ for all $\mathcal C$}{
            %         $i \gets i+1$\\
            %     }
            %     \If{$i > \minsup$}{
            %          $F \gets F \cup c$
            %       }
            %   }
            % }
              
            %{\bf end procedure}
\end{algorithm}


==> algorithms/rulediscovery.tex <==
\begin{algorithm}[!t] 
	\caption{Rule discovery}	\label{alg:rulediscovery}
		\DontPrintSemicolon
			    \SetKwInOut{Input}{input}
	            \SetKwInOut{Output}{output}
	             \SetKwFunction{Expand}{Expand}
	          %  \Input{Graph $\graph$, min support $\minsup$, length $\minlen$}
	           % \Output{set of rules}
              %{\bf return} rule;\\
              $\rules \gets \varnothing$\\
               ${\mathcal C} \gets \forall (p \Rightarrow p')$ such that $p,p'$ are unit path patterns $\in \pathpatterns_1 \cup \pathpatterns^*$\\
                \While{${\mathcal C} \neq \varnothing$}{
            %   \For{$c \in \mathcal C$}{
            %   $i \gets 0$\\
            %   \For{$v \in V$}{
            %         \If{$A(v) \subseteq c$}{
            %             $i \gets i+1$\\
            %         }
            %       }
            %       \If{$i > \minsup$}{
            %          $F \gets F \cup c$
            %       }
            %       }
                  $\rules \gets \rules \cup$ {\sf Discovery(${\mathcal C}, \graph, \minsup$)}\\
                  ${\mathcal C} \gets \forall (p \Rightarrow p')$ so that either $p$ or $p'$ are horizontally and vertically extended path patterns in $\rules$.\\
              }
               
               
            %       \For{$c, c' \in \mathcal C$}{
            %       $i \gets 0$\\
            %       \For{$\elabel \in \mathcal N$}{
                  
            %         \For{$v \in V$}{
            %             \If{$A(v) \subseteq c$ and $A(v')$}{
            %                 $i \gets i+1$\\
            %             }
            %           }
                     
            %           \If{$i > \minsup$}{
            %              $F \gets F \cup c$
            %           }
            %       }
            %   }
            %   \While{1}{
            %       ${\mathcal C} \gets$ {\sf ExtendCandidate($F$)}\\
            %       \If{$\mathcal C = \varnothing$}{\bf{break}}                 
                  
            %       \For{$v \in V$}{
            %          \If{$v.F \subseteq c$ for all $\mathcal C$}{
            %             $i \gets i+1$\\
            %         }
            %         \If{$i > \minsup$}{
            %              $F \gets F \cup c$
            %           }
            %       }
            %   }
              
              {\sf ComputeMetrics}$(\rules)$\\
              %{\bf end procedure}
\end{algorithm}


==> algorithms/simplepathdiscovery.tex <==
\begin{algorithm}[!t] 
	\caption{Frequent simple path pattern discovery}	\label{alg:simplepathpattern}
		\DontPrintSemicolon
			    \SetKwInOut{Input}{input}
	            \SetKwInOut{Output}{output}
	             \SetKwFunction{Expand}{Expand}
	            %\Input{Graph $\graph$, min support $\minsup$, length $\minlen$}
              
              \For{$i = 1$ to $k$}{
                   $\pathpatterns_{i} \gets \varnothing$\\
                  ${\mathcal C} \gets ${\sf VerticalExtend(${\pathpatterns}_{i-1}$)\\       
                  \While{${\mathcal C} \neq \varnothing$}{
            %   \For{$c \in \mathcal C$}{
            %   $i \gets 0$\\
            %   \For{$v \in V$}{
            %         \If{$A(v) \subseteq c$}{
            %             $i \gets i+1$\\
            %         }
            %       }
            %       \If{$i > \minsup$}{
            %          $F \gets F \cup c$
            %       }
            %       }
                  ${\pathpatterns}_i \gets {\pathpatterns}_i \cup$ {\sf Discovery(${\mathcal C}, \graph, \minsup$)}\\
                  ${\mathcal C} \gets$ {\sf HorizontalExtend(${\pathpatterns}_i$)}\\
                }
                }   
                }
        
                                 
            %       \While{1}{
            %       ${\mathcal C} \gets$ {\sf GenerateCandidate($F$)}\\
            %       \If{$\mathcal C = \varnothing$}{\bf{break}}
                  
            %       \For{$v \in V$}{
            %          \If{$v.F \subseteq c$ for all $\mathcal C$}{
            %             $i \gets i+1$\\
            %         }
            %         \If{$i > \minsup$}{
            %              $F \gets F \cup c$
            %           }
            %       }
                  
            %     }
            %   }
             % {\bf end procedure}
\end{algorithm}

